About Synchronized Globular Cluster Formation over Supra-galactic Scales

Observational and theoretical arguments support the idea that violent events connected with $AGN$ activity and/or intense star forming episodes have played a significant role in the early phases of galaxy formation at high red shifts. Being old stellar systems, globular clusters seem adequate candidates to search for the eventual signatures that might have been left by those energetic phenomena. The analysis of the colour distributions of several thousands of globular clusters in the Virgo and Fornax galaxy clusters reveals the existence of some interesting and previously undetected features. A simple pattern recognition technique, indicates the presence of "colour modulations", distinctive for each galaxy cluster. The results suggest that the globular cluster formation process has not been completely stochastic but, rather, included a significant fraction of globulars that formed in a synchronized way and over supra-galactic spatial scales.

==> abstract.tex <==
 
 Observational and theoretical arguments support the idea that violent
 events connected with $AGN$ activity and/or intense star forming episodes
 have played a significant role in the early phases of galaxy formation at
 high red shifts. Being old stellar systems, globular clusters seem
 adequate candidates to search for the eventual signatures that might
 have been left by those energetic phenomena. The analysis of the
 colour distributions of several thousands of globular clusters in the
 Virgo and Fornax galaxy clusters reveals the existence of some 
 interesting and previously undetected features. A simple pattern recognition
 technique, indicates the presence of "colour modulations", distinctive for
 each galaxy cluster. The results suggest that the globular cluster formation 
 process has not been completely stochastic but, rather, included a significant
 fraction of globulars that formed in a synchronized way and over supra-galactic 
 spatial scales.   


